The distribution amplitude of the $\eta_c$-meson

In this proceeding we determine the distribution amplitude of the $\eta_c$-meson from first principles. This quantity appears as a consequence of factorization theorems, and it is necessary to compute the amplitude of multiple exclusive processes. Since it is defined along a light-cone, its calculation via lattice QCD was impossible until recently, when a generalization to Euclidean metric was proposed, and a connection to the physical limit was established. We briefly explain the method of short distance factorization, which allows us to compute the distribution amplitude, and our lattice setup. After summarizing the steps for the continuum and chiral extrapolation, we present our results and compare them to two alternative determinations, one using non-relativistic QCD and another solving the Dyson-Schwinger equations; we find a large discrepancy with the former.

==> tables/cls-ensembles.tex <==
\begin{tabular}{lccc cc ccc}
\toprule
  id &
  $\beta$ &
  $a~[\unit{\femto\metre}]$ &
  $L/a$ &
  $am_{\Ppi}$ &
  $m_{\Ppi}~[\unit{\mega\eV}]$ &
  $m_{\Ppi}L$ &
  $\kappa_{\Pcharm}$ &
  Measurements \\
\midrule
  A5  & 5.2 & 0.0755(9)(7) & $32$ & \num{0.1265(8)} & 331 & 4.0 & 0.12531 & 1980 \\
  B6  &     &              & $48$ & \num{0.1073(7)} & 281 & 5.2 & 0.12529 & 1180 \\
\midrule
  D5* & 5.3 & 0.0658(7)(7) & $24$ & \num{0.1499(1)} & 449 & 3.6 & 0.12724 & 1500 \\
  E5  &     &              & $32$ & \num{0.1458(3)} & 437 & 4.7 & 0.12724 & 2000 \\
  F6  &     &              & $48$ & \num{0.1036(3)} & 311 & 5.0 & 0.12713 & 1200 \\
  F7  &     &              & $48$ & \num{0.0885(3)} & 265 & 4.3 & 0.12713 & 2000 \\
  G8  &     &              & $64$ & \num{0.0617(3)} & 185 & 4.1 & 0.12710 & 1790 \\
\midrule
  N6  & 5.5 & 0.0486(4)(5) & $48$ & \num{0.0838(2)} & 340 & 4.0 & 0.13026 & 1900 \\
  O7  &     &              & $64$ & \num{0.0660(1)} & 268 & 4.2 & 0.13022 & 1640 \\
\bottomrule
\end{tabular}

==> tables/moments.tex <==
\begin{tabular}{c ccc}
\toprule
                & This work      & DB              & NRQCD       \\
$\expval*{g^2}$ & \num{0.134(6)} & \num{0.118(18)} & \num{0.171(23)}    \\
$\expval*{g^4}$ & \num{0.043(4)} & \num{0.036(9)}  & \num{0.018808(19)} \\
\bottomrule
\end{tabular}


==> tables/results.tex <==
\begin{tabular}{crrr}
    \toprule
    $\lambda$ & $2.73\pm0.12\pm0.12\pm0.06$       & $2.75\pm0.12$      & $2.61\pm0.15$      \\
    $a_{1,2}$ & $-7.58\pm0.05\pm0.59\pm0.55$      & $-8.12\pm0.05$     & $-8.68\pm0.13$     \\
    $b_{1,2}$ & $0.88\pm0.07\pm0.08\pm0.06$       & $0.89\pm0.07$      & $0.77\pm0.10$      \\
    $c_{1,2}$ & $-0.042\pm0.002\pm0.005\pm0.001$  & $-0.0428\pm0.0022$ & $-0.0440\pm0.0028$ \\
    $d_{1,2}$ & $-2.221\pm0.015\pm0.063\pm0.15$   & $-2.368\pm0.015$   & $-2.52\pm0.04$     \\
    $e_{1,2}$ & $-0.0897\pm0.001\pm0.159\pm0.116$ & $-0.1700\pm0.0016$ & $-0.321\pm0.005$   \\
    \bottomrule
\end{tabular}
